Predictive Process Monitoring Methods: Which One Suits Me Best?

Predictive process monitoring has recently gained traction in academia and is maturing also in companies. However, with the growing body of research, it might be daunting for companies to navigate in this domain in order to find, provided certain data, what can be predicted and what methods to use. The main objective of this paper is developing a value-driven framework for classifying existing work on predictive process monitoring. This objective is achieved by systematically identifying, categorizing, and analyzing existing approaches for predictive process monitoring. The review is then used to develop a value-driven framework that can support organizations to navigate in the predictive process monitoring field and help them to find value and exploit the opportunities enabled by these analysis techniques.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

==> usecase.tex <==
\subsection{Datasets}
\label{ssec:dataset}
For the tool evaluation, we used two datasets provided for the BPI Challenges 2011~\cite{bpichallenge2011} and 2015~\cite{bpichallenge2015}, respectively.

The first event log pertains to the treatment of patients diagnosed with cancer in a large Dutch Academic Hospital. It contains 1,140 traces, 149,730 events referring to 623 different activities.
In this case, we used our framework to predict the information that, for example, \emph{Bob} is interested to know about the \emph{Alice}'s case (see \emph{Scenario 1} in Section~\ref{sec:scenarios}). More formally, we used our framework to predict the compliance of a trace with respect to the following two LTL rules:
\begin{itemize}\scriptsize
\scriptsize
  \item $\varphi_{11} = \lfuture(``tumor~marker~CA-19.9") \vee  \lfuture(``ca-125~using~meia")$,
  \item $\varphi_{12} = \lglobally(``CEA-tumor~marker~using~meia" \rightarrow$   $\lfuture(``squamous~cell~carcinoma~using~eia"))$.
\end{itemize}

The second log was provided by a Dutch Municipality. The log is composed of 1,199 traces, 52,217 events and 398 event classes.  The data contains all building permit applications over a period of approximately four years. It contains several activities, denoted by both codes and labels, both in Dutch and in English.
%
In this case, we used the \premoplus to investigate the configurations that are more suitable with respect to the \emph{John}'s problem (see \emph{Scenario 2} in Section~\ref{sec:scenarios}). Formally, we investigate the following two LTL rules:
\begin{itemize}\scriptsize
\scriptsize
  \item $\varphi_{21} = (\lfuture(``start~WABO~procedure'') \wedge \lfuture(``extend~procedure~term''))$,
  \item $\varphi_{22} = (\lglobally(``send~confirmation~receipt'')  \rightarrow$   $\lfuture(``retrieve~missing~data"))$.
\end{itemize}


